How To Think About End-To-End Encryption and AI: Training, Processing, Disclosure, and Consent

End-to-end encryption (E2EE) has become the gold standard for securing communications, bringing strong confidentiality and privacy guarantees to billions of users worldwide. However, the current push towards widespread integration of artificial intelligence (AI) models, including in E2EE systems, raises some serious security concerns. This work performs a critical examination of the (in)compatibility of AI models and E2EE applications. We explore this on two fronts: (1) the integration of AI "assistants" within E2EE applications, and (2) the use of E2EE data for training AI models. We analyze the potential security implications of each, and identify conflicts with the security guarantees of E2EE. Then, we analyze legal implications of integrating AI models in E2EE applications, given how AI integration can undermine the confidentiality that E2EE promises. Finally, we offer a list of detailed recommendations based on our technical and legal analyses, including: technical design choices that must be prioritized to uphold E2EE security; how service providers must accurately represent E2EE security; and best practices for the default behavior of AI features and for requesting user consent. We hope this paper catalyzes an informed conversation on the tensions that arise between the brisk deployment of AI and the security offered by E2EE, and guides the responsible development of new AI features.

==> e2ee-properties.tex <==
\subsection{Key properties of E2EE endangered by AI}
\label{sec:background:e2ee-properties}
%

%

%

In this section, we present critical security considerations for E2EE systems that are endangered by AI assistants.
We distinguish between two types of guarantees: \emph{individual guarantees}, which are promises about the confidentiality of the data from each user; and \emph{systemic guarantees}, which are broader promises about the confidentiality of the entire E2EE ecosystem.


\paragraph{Individual privacy considerations} Individual guarantees concern only individual users, irrespective of the behavior or state of any other users in the system.
E2EE applications provide three core individual guarantees \cite{e2ee-definition-rfc}:
\begin{newitemize}
    \item \emph{Message confidentiality}: Plaintext messages can only be seen by the sender and intended recipients; no one else---including state-level adversaries, or the service provider itself---can intercept or monitor communications.
    \item \emph{Message integrity}: Plaintext messages cannot be tampered with in ways that would go undetected.
    \item \emph{Message authenticity}: Users of the system can prove their identities to, and verify the identities of, other users in the system.
\end{newitemize}
Together, these three properties guarantee that, for any user of the system, their messages will not be read (confidentiality) nor undetectibly smodified (integrity), and they will not be impersonated (authenticity).
Besides these core guarantees, E2EE applications generally provide additional auxiliary security features, which have come to be expected of modern E2EE applications.
One example is \emph{forward secrecy}, which states that an adversary who has compromised one of the core properties (e.g., by stealing the victims' secret key) cannot violate the guarantees for messages that were transmitted before the compromise; conversely, \emph{post-compromise security} states that an adversary that has compromised one of the core properties cannot violate the guarantees for messages that are transmitted after the protocol ``heals'' itself (e.g., sampling a new secret key for the victim). %

%

\paragraph{Systemic privacy considerations} Beyond individual privacy guarantees, E2EE applications offer systemic guarantees for being part of the user set for the E2EE application.
The most critical property is \emph{unincriminatingness}, which states that usage of the E2EE system (over alternative messaging systems, or a non-E2EE version of the same system) is not considered remarkable.
What this property seeks to capture is the idea that using the E2EE application should not be \emph{ipso facto} incriminating; by necessity this property is not wholly determined by the technical configuration of a system, but is instead socially-determined, emergent, and contextual.

Illustrating the significance and definition of this property may be best clarified by providing examples of systems which \emph{lack} this property.


